Optimal Nonparametric Inference with Two-Scale Distributional Nearest Neighbors

The weighted nearest neighbors (WNN) estimator has been popularly used as a flexible and easy-to-implement nonparametric tool for mean regression estimation. The bagging technique is an elegant way to form WNN estimators with weights automatically generated to the nearest neighbors; we name the resulting estimator as the distributional nearest neighbors (DNN) for easy reference. Yet, there is a lack of distributional results for such estimator, limiting its application to statistical inference. Moreover, when the mean regression function has higher-order smoothness, DNN does not achieve the optimal nonparametric convergence rate, mainly because of the bias issue. In this work, we provide an in-depth technical analysis of the DNN, based on which we suggest a bias reduction approach for the DNN estimator by linearly combining two DNN estimators with different subsampling scales, resulting in the novel two-scale DNN (TDNN) estimator. The two-scale DNN estimator has an equivalent representation of WNN with weights admitting explicit forms and some being negative. We prove that, thanks to the use of negative weights, the two-scale DNN estimator enjoys the optimal nonparametric rate of convergence in estimating the regression function under the fourth-order smoothness condition. We further go beyond estimation and establish that the DNN and two-scale DNN are both asymptotically normal as the subsampling scales and sample size diverge to infinity. For the practical implementation, we also provide variance estimators and a distribution estimator using the jackknife and bootstrap techniques for the two-scale DNN. These estimators can be exploited for constructing valid confidence intervals for nonparametric inference of the regression function. The theoretical results and appealing finite-sample performance of the suggested two-scale DNN method are illustrated with several numerical examples.

==> figures_tables/setting_1_normal_fixed_results_table.tex <==

\begin{tabular}{lccccc}
\toprule
Method & MSE & Bias & Variance & True Mean & Est. Mean (SE)\\
\midrule
DNN & 0.1287 & 0.2389 & 0.0629 & -1.125 & -0.8861 (0.2677)\\
k-NN & 0.3328 & 0.0989 & 0.3183 & -1.125 & -1.0261 (0.5686)\\
TDNN & 0.0988 & -0.0574 & 6.4475 & -1.125 & -1.1824 (0.3091)\\
\bottomrule
\end{tabular}


==> figures_tables/setting_1_normal_random_results_table.tex <==

\begin{tabular}{lccc}
\toprule
Method & MSE & Bias & Variance\\
\midrule
DNN & 15.1659 & -0.8013 & 0.5974\\
k-NN & 9.5352 & -0.5137 & 2.2475\\
TDNN & 7.2606 & -0.4862 & 1.5662\\
\bottomrule
\end{tabular}


==> figures_tables/setting_1_unif_fixed_results_table.tex <==

\begin{tabular}{lccccc}
\toprule
Method & MSE & Bias & Variance & True Mean & Est. Mean (SE)\\
\midrule
DNN & 0.0389 & 0.0643 & 0.0265 & 2.125 & 2.1893 (0.1865)\\
k-NN & 0.0500 & 0.0445 & 0.0467 & 2.125 & 2.1695 (0.2192)\\
TDNN & 0.0263 & 0.0165 & 0.0253 & 2.125 & 2.1415 (0.1613)\\
\bottomrule
\end{tabular}


==> figures_tables/setting_1_unif_random_results_table.tex <==

\begin{tabular}{lccc}
\toprule
Method & MSE & Bias & Variance\\
\midrule
DNN & 0.1340 & -0.0547 & 0.0405\\
k-NN & 0.1824 & -0.0940 & 0.0496\\
TDNN & 0.1302 & -0.0489 & 0.0652\\
\bottomrule
\end{tabular}


==> figures_tables/setting_2_fixed_results_table.tex <==

\begin{tabular}{lcccccc}
\toprule
Method & p & MSE & Bias & Variance & True Mean & Est. Mean (SE)\\
\midrule
DNN & 3 & 0.0326 & -0.0186 & 0.0261 & 0.6582 & 0.6396 (0.1796)\\
k-NN & 3 & 0.1696 & -0.0210 & 0.1764 & 0.6582 & 0.6372 (0.4115)\\
TDNN & 3 & 0.0235 & -0.0174 & 0.0219 & 0.6582 & 0.6408 (0.1525)\\
\addlinespace
DNN & 5 & 0.0349 & -0.0133 & 0.0249 & 0.6582 & 0.6449 (0.1863)\\
k-NN & 5 & 0.1480 & -0.0374 & 0.1505 & 0.6582 & 0.6208 (0.3831)\\
TDNN & 5 & 0.0238 & -0.0202 & 0.0223 & 0.6582 & 0.638 (0.1531)\\
\addlinespace
DNN & 10 & 0.0314 & -0.0170 & 0.0245 & 0.6582 & 0.6412 (0.1764)\\
k-NN & 10 & 0.0856 & -0.0282 & 0.0838 & 0.6582 & 0.63 (0.2914)\\
TDNN & 10 & 0.0244 & -0.0157 & 0.0226 & 0.6582 & 0.6425 (0.1556)\\
\addlinespace
DNN & 15 & 0.0360 & -0.0083 & 0.0258 & 0.6582 & 0.6498 (0.1897)\\
k-NN & 15 & 0.0521 & -0.0383 & 0.0515 & 0.6582 & 0.6199 (0.2251)\\
TDNN & 15 & 0.0251 & -0.0146 & 0.0235 & 0.6582 & 0.6436 (0.1579)\\
\addlinespace
DNN & 20 & 0.0319 & -0.0075 & 0.0262 & 0.6582 & 0.6507 (0.1786)\\
k-NN & 20 & 0.0425 & -0.0638 & 0.0383 & 0.6582 & 0.5944 (0.1961)\\
TDNN & 20 & 0.0242 & -0.0105 & 0.0231 & 0.6582 & 0.6477 (0.1553)\\
\bottomrule
\end{tabular}


==> figures_tables/setting_2_random_results_table.tex <==

\begin{tabular}{lcccc}
\toprule
Method & p & MSE & Bias & Variance\\
\midrule
DNN & 3 & 2.8799 & 0.4892 & 0.0869\\
k-NN & 3 & 2.2335 & 0.4050 & 0.3126\\
TDNN & 3 & 1.6259 & 0.3016 & 0.2586\\
\addlinespace
DNN & 5 & 2.9039 & 0.4932 & 0.0867\\
k-NN & 5 & 3.8489 & 0.5610 & 0.2953\\
TDNN & 5 & 1.6539 & 0.3069 & 0.2608\\
\addlinespace
DNN & 10 & 2.9509 & 0.4953 & 0.0861\\
k-NN & 10 & 5.0886 & 0.6142 & 0.1611\\
TDNN & 10 & 1.6991 & 0.3119 & 0.2600\\
\addlinespace
DNN & 15 & 2.9461 & 0.4961 & 0.0871\\
k-NN & 15 & 5.4081 & 0.6091 & 0.0960\\
TDNN & 15 & 1.6893 & 0.3103 & 0.2673\\
\addlinespace
DNN & 20 & 2.9576 & 0.4966 & 0.0868\\
k-NN & 20 & 5.5638 & 0.5872 & 0.0693\\
TDNN & 20 & 1.7022 & 0.3125 & 0.2661\\
\bottomrule
\end{tabular}

